Deformations of pullback foliations

We study the stability of pullback foliations under morphisms and rational maps via Grothendieck's Drapeaux scheme. In the local setting, a foliated version of Schlessinger's Theorem on rigidity of conical singularities was achieved. We apply these techniques to provide a criterion for the stability of algebraic leaves of a foliation.

==> Chapters/Translation.tex <==
\section{Deformations of pullbacks under morphisms}

\begin{definition}
Let $\X/S$ and $\Y/S$ be considered two locally trivial families of normal manifolds, $\Pi: \X\rightarrow \Y$ an $S$-map and $\dG/S$ is a family of integrable distributions on $\Y/S$. The \textit{pullback} $\dF/S = \Pi^\ast(\dG/S)$ is defined as that family of integrable distributions on $\X/S$ whose tangent subbundle $T_{\dF/S}$ is the kernel of the composition
\[
T_{\X/S}\rightarrow \Pi^{[\ast]} T_{\Y/S}\rightarrow \Pi^{[\ast]} N_{\dG/S}.
\]
\end{definition}

It should be noted that since $\Pi^{[\ast]} N_{\dG/S}$ is the dual of a sheaf it has to be torsionless, and hence the normal $N_{\dF/S}$ is also torsionless since it is a subsheaf of the former. We are now in a position to state the main result of this chapter:

\begin{theorem}{\label{stability_morphisms}}
Consider a morphism $\pi: X\rightarrow Y$ between normal manifolds that is proper, surjective, with connected fibers and whose generic fiber is smooth and has no global $1$-forms. Suppose that
\[
0\rightarrow T_{\dF/S}\rightarrow T_{\X/S}\rightarrow N_{\dF/S}\rightarrow 0
\]
is a deformation of a pullback foliation $\F = \pi^\ast\G = \dF_s$ with smooth basis $S$. If the family $\X$ is projective on $S$ and $\Pi: \X\rightarrow \Y$ is a deformation of $\pi$ on $S$, then there exists an epicentre $U\rightarrow S$ of $s$ and a deformation $\dG/U$ of $\G = \dG_s$ such that $\dF/U = \Pi^\ast(\dG/U)$.
\end{theorem}

In order to prove it, we first need the following vanishing lemma:

\begin{lemma}{\label{vanishing}}
Let $\pi: X\rightarrow Y$ be a proper morphism between normal manifolds such that its generic fiber is smooth and it has no global 1-forms. If $\F = \pi^\ast\G$ is a pullback foliation, then $\Hom(T_{X/Y},N_\F) = 0$.
\end{lemma}

\begin{proof}
Note that since $N_\F$ is torsion-free, then $\sHom(T_{X/Y},N_\F)$ is also torsion-free. So if we want to prove that the global sections of this last sheaf are null, it will suffice to verify that such sections are generically null. This allows us to assume, after restricting ourselves to an appropriate open set of $X$, that the manifolds involved, the morphism $\pi$ and the foliation $\G$ are smooth. Thus the normal bundle of $\F$ turns out to be equal to $N_\F =\pi^\ast N_\G$. Going through a smaller open set again if necessary we can assume that $N_\G = \OO_{Y}^{q}$. On the other hand, thanks to the hypothesis about fibers and \cite[Cohomology and Base Change Theorem]{vakil2017rising} we can conclude that $\pi_\ast\Omega^1_{X/Y} = 0$, with which
\[
\Hom(T_{X/Y},N_\F) = \Gamma\big(\Omega_{X/Y}^1\big)^q = \Gamma\big(\pi_\ast\Omega^1_{X/Y}\big)^q = 0
\]
as we wanted to prove. \end{proof}

In particular, if we specialize this lemma to the case where $\G$ is the point foliation, we obtain the following result on rigidity of foliations given by fibrations...

\begin{corollary}{\label{rigidity}}
If $\F$ is the foliation whose leaves are the fibers of a proper morphism $\pi: X\rightarrow Y$ with smooth generic fiber and no global 1-forms, then the tangent $T_\F = T_{X/Y}$ is rigid as a subbundle of $T_X$.
\end{corollary}

%\textcolor{purple}{Conjetura: Si $\pi: X\rightarrow Y$ es suave y $H^0(T_Y) = 0$, entonces $\Hom(T_{X/Y},\pi^\ast T_Y) = 0$. Conozco dos instancias en las que vale esto: si $X$ es un producto, y si $X$ es una fibración elíptica suave (ver mis notas, usa el grado de la imagen directa del anticanónico) }


\begin{proof}[Proof of Theorem \ref{stability_morphisms}]
Note that the coherent bundle $\E = T_{\X/S}$ is flat over $S$, so the choice of an $S$-wide bundle $\OO_\X(1)$ allows us to construct the schemes $\Drap_\E$ and $\Quot_\E$. Let $p\in \Drap_{\E}$ be the point on $s\in S$ corresponding to the filtration
\[
T_{X/Y}\subseteq T_{\F}\subseteq T_{X} = \E|_s.
\]
Thanks to the \ref{vanishing} Lemma we know that condition (a) of Proposition \ref{smooth} is verified. In turn, the subbundle $T_{\X/\Y}\subseteq \E$ corresponds to a section $S\rightarrow \Quot_\E$ of a structural morphism $\Quot_{\E}\rightarrow S$ whose image contains the point $\varphi_1(p)$, and hence condition (b) is a consequence of the Corollary \ref{rigidity} and the smoothness of $S$. Similarly, the inclusion $T_{\dF/S}\subseteq \E$ corresponds to a section $\sigma:S\rightarrow \Quot_{\E}$ of the structural morphism such that $\sigma(s) = \varphi_2(p)$. Using \cite[Corollaire 17.16.3]{EGAIV.4} we can find an étale neighborhood $U\rightarrow S$ of $s$ and a survey $\widetilde{\sigma}: U\rightarrow\Drap_{\E}$ that commutes the diagram \begin{center} \begin{tikzcd}[column sep = 25 pt, row sep = 20 pt] U \arrow[r, {\sigma}"] \arrow[d] & \Drap_\E \arrow[d, "\varphi_2"] \\ S\arrow[r, "\sigma"'] & \Quot_\E \end{tikzcd} \end{center} such that there exists $u\in U$ with $\widetilde{\sigma}(u) = p$. The morphism $\widetilde{\sigma}:U\rightarrow\Drap_\E$ corresponds to a filtration $F_1\subseteq T_{\dF/U} \subseteq T_{\X/U}$. By the rigidity of $T_{X/Y}$ we can affirm after replacing $U$ by a smaller neighborhood that $F_1 = T_{\X/\Y}|_U$. The result follows from Lemma \ref{jorge}.
\end{proof}

==> Preamble/style.tex <==
% Formato del título de capítulos y secciones
\titleformat{\chapter}[block]{\normalfont\huge\bfseries}{\thechapter.}{.5em}{\huge}[\vspace{2pt}{\titlerule[2pt]}]

\titlespacing*{\chapter}{0pt}{-19pt}{25pt}

\titleformat{\section}[block]{\normalfont\Large\bfseries}{\thesection.}{.5em}{\Large}

\titleformat{\part}[block]{\titlerule[2pt]\normalfont\Huge\bfseries\centering}{Parte \Roman{part}\\\vspace{15pt}}{0pt}{\Huge}[\vspace{2pt}{\titlerule[2pt]}]

% Tamaños y estilos de elementos en la TOC
\DeclareTOCStyleEntry[
    linefill=\bfseries\TOCLineLeaderFill,
    beforeskip=12pt,
    entrynumberformat=\chapterprefixintoc,
    entryformat=\chaptertocformat,
    pagenumberformat=\chaptertocformat,
    dynnumwidth
]{tocline}{chapter}

\DeclareTOCStyleEntry[
    % linefill=\bfseries\TOCLineLeaderFill,
    beforeskip=30pt,
    entrynumberformat=\chapterprefixintoc,
    entryformat=\parttocformat,
    pagenumberformat=\partpagetocformat,
    numwidth=0pt
]{tocline}{part}

\newcommand\chaptertocformat[1]{\large{\textbf{#1}}}%
\newcommand\chapterprefixintoc[1]{#1}%
\newcommand\parttocformat[1]{\Large{\textbf{#1}}}%
\newcommand\partpagetocformat[1]{} % Don't print the page number for parts

% Alias para estilos de texto comunes
\newcommand{\negritas}[1]{\textbf{#1}}
\newcommand{\cursiva}[1]{\textit{#1}}
\newcommand{\codigo}[1]{\texttt{#1}}

% Formato del código fuente con lstlisting
\lstset{
  basicstyle=\ttfamily,
  breaklines=true,
}

% Márgenes
\geometry{
    a4paper,
    margin=2.5cm
}
\setlength{\marginparwidth}{2cm} 

% Limite de profundidad del índice
\setcounter{tocdepth}{2}

% Eliminar el guionado
%\tolerance=1
%\emergencystretch=\maxdimen
%\hyphenpenalty=10000
%\hbadness=10000

% Indentación de párrafos
\setlength{\parindent}{.75cm}

\renewcommand{\lstlistingname}{Extracto de código}
\renewcommand*{\lstlistlistingname}{Índice de extractos de código}

% Comandos para establecer variables
\newcommand{\setTitle}[1]{\def\tfgTitle {#1}}
\newcommand{\setAuthor}[1]{\def\tfgAuthors {#1}}
\newcommand{\setDegree}[1]{\def\tfgDegree {#1}}
\newcommand{\setSupervisor}[1]{\def\tfgSupervisor {#1}}
\newcommand{\setDepartment}[1]{\def\tfgDepartment {#1}}
\newcommand{\setMonth}[1]{\def\tfgMonth {#1}}
\newcommand{\setYear}[1]{\def\tfgYear {#1}}
\newcommand{\setDedication}[1]{\def\tfgDedication {#1}}

% Estilos para el código
% Configuración genérica
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{editorOcher}{rgb}{0.8, 0.3, 0} % #FF7F00 -> rgb(239, 169, 0)
\definecolor{editorGreen}{rgb}{0, 0.5, 0} % #007C00 -> rgb(0, 124, 0)

\lstdefinestyle{listingstyle}{
    backgroundcolor=\color{white},  
    keywordstyle=\bfseries\color{blue},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{editorGreen},
    commentstyle=\color{codegray},
    basicstyle=\ttfamily\color{black},
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2,
    frame=tb,
    keywords=[2]{True,False},
    literate=%
*{0}{{{\color{editorOcher}0}}}1
{1}{{{\color{editorOcher}1}}}1
{2}{{{\color{editorOcher}2}}}1
{3}{{{\color{editorOcher}3}}}1
{4}{{{\color{editorOcher}4}}}1
{5}{{{\color{editorOcher}5}}}1
{6}{{{\color{editorOcher}6}}}1
{7}{{{\color{editorOcher}7}}}1
{8}{{{\color{editorOcher}8}}}1
{9}{{{\color{editorOcher}9}}}1,
}

\lstset{style=listingstyle}
\lstset{columns=fullflexible}


